Garbage Collection for Multicore NUMA Machines

Modern high-end machines feature multiple processor packages, each of which contains multiple independent cores and integrated memory controllers connected directly to dedicated physical RAM. These packages are connected via a shared bus, creating a system with a heterogeneous memory hierarchy. Since this shared bus has less bandwidth than the sum of the links to memory, aggregate memory bandwidth is higher when parallel threads all access memory local to their processor package than when they access memory attached to a remote package. This bandwidth limitation has traditionally limited the scalability of modern functional language implementations, which seldom scale well past 8 cores, even on small benchmarks. This work presents a garbage collector integrated with our strict, parallel functional language implementation, Manticore, and shows that it scales effectively on both a 48-core AMD Opteron machine and a 32-core Intel Xeon machine.

==> common/lstlang-bomil.tex <==
\lstdefinelanguage{BOMIL}{%
  morekeywords={%
    addr, alloc, and, any, apply, bool, byte, case, ccall, cont, define, do, double,%
    enum, extern, false, float, fun, host_vproc, if, inline, int, let, long, module,%
    noreturn, promote, pure, return, short, tag, throw, true, typedef, unwrap, use_rw,%
    vec128, void, vproc, vpload, vpstore, wrap,%
  },%
  keywordsprefix=@,
  % otherkeywords={(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  sensitive,%
  morecomment=[n]{(*}{*)},%
  morestring=[d]",%
}[keywords,comments,strings]%


==> common/lstlang-manticore.tex <==
\lstdefinelanguage{Manticore}[]{SML}{%
  morekeywords={by,otherwise,pcase,pval,spawn,to},
  % otherkeywords={(|,|),[|,|],(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  otherkeywords={(|,|),[|,|],?,\&},
}[keywords,comments,strings]%


==> common/lstlang-sml.tex <==
\lstdefinelanguage{SML}{%
  morekeywords={%
    abstype, and, andalso, as, case, datatype, do, else, end, eqtype, exception,%
    fn, fun, functor, handle, if, in, include, infix, infixr, let, local, nonfix,%
    of, op, open, orelse, raise, rec, sharing, sig, signature, struct, structure,%
    then, type, val, where, while, with, withtype,%
  },%
  % otherkeywords={(,),[,],\{,\},\,,:,...,_,|,=,=>,->,\#,:>},
  sensitive,%
  morecomment=[n]{(*}{*)},%
  morestring=[d]",%
}[keywords,comments,strings]%


==> common/slide-defs.tex <==
% slide-defs.tex
%
% common definitions for talks.
%
% define \TalkDate and \TalkTitle for footers
%

% for a 1024x768 screen, we have a 1.0:0.75 ratio.
\setlength{\textwidth}{9.3in}
\setlength{\textheight}{7.2in}
\addtolength{\leftmargin}{-0.15in}
\addtolength{\topmargin}{-0.7in}

\usepackage{color}
\usepackage{graphicx}
\usepackage{times}

%
% the following magic makes the tt font in math mode be the same as the
% normal tt font (i.e., Courier)
%
\SetMathAlphabet{\mathtt}{normal}{OT1}{pcr}{n}{n}
\SetMathAlphabet{\mathtt}{bold}{OT1}{pcr}{bx}{n}

\definecolor{Red}{rgb}{0.8,0.0,0.0}
\definecolor{Green}{rgb}{0.0,0.4,0.0}
\definecolor{Blue}{rgb}{0.0,0.0,0.9}
\definecolor{Purple}{rgb}{0.5,0.0,0.4}
\definecolor{Black}{rgb}{0.0,0.0,0.0}
\definecolor{Yellow}{rgb}{1.0,1.0, 0.25}
\definecolor{Cyan}{rgb}{0.25,1.0, 1.0}
\newcommand{\blue}[1]{\color{Blue}{#1}}
\newcommand{\red}[1]{\color{Red}{#1}}
\newcommand{\green}[1]{\color{Green}{#1}}
\newcommand{\purple}[1]{\color{Purple}{#1}}
\newcommand{\textblue}[1]{\textcolor{Blue}{#1}}
\newcommand{\textred}[1]{\textcolor{Red}{#1}}
\newcommand{\textgreen}[1]{\textcolor{Green}{#1}}
\newcommand{\textpurple}[1]{\textcolor{Purple}{#1}}
\newcommand{\textblack}[1]{\textcolor{Black}{#1}}

\newcommand{\mobycodecolor}{\color{Purple}}
\newcommand{\punctcolor}{\color{Blue}}
\newcommand{\kwcolor}{\color{Blue}}
\newcommand{\bolcodecolor}{\color{Green}}
\newcommand{\ccodecolor}{\color{Purple}}
%\newcommand{\highlightC}[1]{\textred{#1}}
\newcommand{\highlightC}[1]{\colorbox{Yellow}{#1}}
\newcommand{\highlightCC}[1]{\colorbox{Cyan}{#1}}

\newcommand{\BlueBullet}{\textcolor{Blue}{\ensuremath{\bullet}}}
\newcommand{\RedBullet}{\textcolor{Red}{\ensuremath{\bullet}}}
\newcommand{\GreenBullet}{\textcolor{Green}{\ensuremath{\bullet}}}

\newcommand{\EM}[1]{\emph{\textred{#1}}}

\raggedright
\pagestyle{empty}

\newcommand{\HEAD}[1]{
  \noindent{\large\bf{}#1}\\[-1ex]
  \textblue{\hrulefill}\\[1em]}
\newcommand{\CONTINUE}[1]{
  \noindent{\bf{}#1 {\it{}(continued ...)}}\\[-1ex]
   \textblue{\hrulefill}\\[1em]}
\newcommand{\CHEAD}[1]{{\makebox[\textwidth]{\large\bf{}#1}\\[1em]}}
\newcommand{\FOOT}{%
  \vfill\textblue{\hrulefill}\\ %
  \tiny{
    \mbox{\rule[-.5ex]{0em}{3ex}} %
    \TalkDate  \hfill \TalkTitle \hfill \arabic{slide}}%
}

\newenvironment{FIGURE}{%
  \begin{center}\small}{%
  \end{center}}

% code
\newcommand{\tkw}[1]{\text{\kw{#1}}}
\newcommand{\tcd}[1]{\text{\cd{#1}}}
 

==> numa.tex <==
%!TEX root = paper.tex


\section{Measuring NUMA effects}
\label{sec:numa}

In \secref{intro:amdhardware}, we described the exact hardware configuration and 
memory topology of our 48~core AMD Opteron system.
We also described the 32~core Intel Xeon system in
\secref{intro:intelhardware}. 
These systems are the subject of the NUMA tests below.

\subsection{STREAM benchmark}
The C language STREAM benchmark~\cite{stream} consists of the four operations
listed in \tblref{numa:stream}. 
These synthetic memory bandwidth tests were originally selected to measure
throughput rates for a set of common operations that had significantly different
performance characteristics on vector machines of the time.
On modern hardware, each of these tests achieve similar bandwidth, as memory is
the primary constraint, not floating-point execution.
The \kw{COPY} test, in particular, is representative of the type of work
performed by a copying garbage collector.

\begin{table}
\begin{center}
\begin{tabular}{r | l}
Name & Code\\
\hline
\kw{COPY} & \lstinline!a[i] = b[i];! \\
\kw{SCALE} & \lstinline!a[i] = s*b[i];! \\
\kw{SUM} & \lstinline!a[i] = b[i]+c[i];! \\
\kw{TRIAD} & \lstinline!a[i] = b[i]+s*c[i];! \\
\end{tabular}
\end{center}
\caption{
Basic operations in the STREAM benchmark.
}
\label{numa:stream}
\end{table}%
The existing STREAM benchmark does not support NUMA awareness for either the
location of the running code or the location of the allocated memory. 
We modified the STREAM benchmark to measure the achievable memory bandwidth for
these operations across several allocation and access configurations.
The baseline STREAM benchmark allocated a large, static vector of \kw{double}
values.\footnote{There is no difference in bandwidth when using \kw{long}
  values.}
Our modifications use pthreads and libnuma to control the number and placement
of each piece of running code and corresponding
memory~\cite{butenhof:pthreads-book,libnuma}.

While the STREAM benchmark's suggested array sizes for each processor are larger
than the L3 cache, the tests do not take into account cache block sizes.
We extended the tests with support for strided accesses to provide a measure of
RAM bandwidth in the case of frequent cache misses.
This strided access support also allows us to measure the latency of memory
access.

\subsection{Bandwidth evaluation}
\figref{numa:evalBandwidth} plots the bandwidth, in MB/s, versus the number of
threads.
Larger bandwidth is better.
The results are for the \kw{COPY} test, but all of the tests were within a small
factor.
Four variants of the STREAM benchmarks were used: 
\begin{enumerate}
\item \emph{Unstrided} accesses memory attached to its own node and uses the
  baseline STREAM strategy of sequential access through the array.
\item \emph{Unstrided+non-NUMA} accesses the array sequentially, but is
  guaranteed to access that memory on another package.
\item \emph{Strided} also accesses local memory, but ensures that each access is
  to a new cache block.
\item \emph{Strided+non-NUMA} strides accesses, and also references memory from
  another package.
\end{enumerate}
NUMA aware versions ensure that accessed memory is allocated on the same node as
the thread of execution and that the thread is pinned to the node, using the
libnuma library~\cite{libnuma}.
To do this, the modified benchmark pins the thread to a particular node and then
uses the libnuma allocation API to guarantee that the memory is allocated on the
same node.
The non-NUMA aware versions also pin each thread to a particular node, but then
explicitly allocate memory using libnuma from an entirely separate package (not
just a separate node on the same package).
When there are less threads than cores, we pin threads to new nodes rather than
densely packing a single node.

\begin{figure}
\centering
AMD Bandwidth\\
\includegraphics[scale=0.6]{data/amd/bandwidth} \\[3em]
Intel Bandwidth\\
\includegraphics[scale=0.6]{data/intel/bandwidth}
\caption{
Bandwidth vs. number of threads on the STREAM benchmark, comparing strided and NUMA configurations.
Larger bandwidth is better.
}
\label{numa:evalBandwidth}
\end{figure}%

It should not be surprising that the unstrided variants exhibit roughly eight
times the bandwidth of their strided versions, as cache blocks on these machines 
are 64~bytes and the \kw{double} values accessed are each 8~bytes.
In the NUMA aware cases, scaling continues almost linearly until eight threads
and increases until the maximum number of available cores on both machines.
On AMD hardware, non-NUMA aware code pays a significant penalty and begins to
lose bandwidth where NUMA aware code does not at 48~cores.
On the Intel hardware the gap between NUMA and non-NUMA aware code is very small
even when the number of threads is the same as the number of cores.
But, the Intel hardware does not offer as much peak usable bandwidth for
NUMA-aware code, peaking near 40,000~MB/s whereas we achieve nearly 55,000~MB/s
on the AMD hardware.

\figref{numa:evalBandwidthByNode} plots the bandwidth against threads again,
but this time divided by the number of active nodes to provide a usage data
relative to the theoretical interconnect bandwidth detailed in
\tblref{numa:amdbandwidth} for the AMD machine and \tblref{numa:intelbandwidth}
for the Intel machine.
Our benchmarks allocate threads sparsely on the nodes. 
Therefore, when there are less than 8~threads on the AMD machine, that is also
the number of active nodes.
On the Intel machine with 4~nodes, when there are less than 4~threads, that is
the number of active nodes.
These graphs show that on both machines there is a significant gap between
the theoretical bandwidth and that achieved by the strided \kw{COPY} stream
benchmark.
It is also clear that there is a significant non-NUMA awareness penalty on the
AMD machine but that penalty is less on the Intel machine.
However, the Intel machine begins to reach saturation at 32~cores, whereas the
NUMA aware AMD machine continues to increase per-node bandwidth up to 48~cores. 

\begin{figure}
\centering
AMD Bandwidth\\
\includegraphics[scale=0.6]{data/amd/bandwidth_by_node} \\[3em]
Intel Bandwidth\\
\includegraphics[scale=0.6]{data/intel/bandwidth_by_node}
\caption{
Bandwidth per node vs. number of threads on the STREAM benchmark, comparing
strided configurations.
Larger bandwidth is better.
}
\label{numa:evalBandwidthByNode}
\end{figure}%

\subsection{Latency evaluation}
\figref{numa:evalLatency} plots the latency times, in nanoseconds, versus the
number of threads.
Smaller latency times are better.
To measure the latency times, we only consider the strided STREAM benchmarks 
to ensure that we are measuring only the time to access RAM, and not the time
to access cache.
As was the case with bandwidth, the AMD machine's NUMA aware tests maintain good
values up to large numbers of processors.
The non-NUMA aware AMD benchmark begins to exhibit high latencies at moderate
numbers of threads.
On the Intel machine, latency numbers remain low until more than 24~cores are in
use, and then the latencies grow similarly for both NUMA aware and non-NUMA
aware code.

On the AMD machine, these benchmarks and evaluations clearly indicate that at
high numbers of threads of executions, poor choices of memory location or code
execution can have significant negative impact on the latency of memory access
and memory bandwidth.
For the Intel machine, memory performance uniformly increases until high numbers
of threads, at which point is uniformly decreases, seeing little effect from
NUMA awareness.
But, none of these effects show up in practice until more than 24~threads are in
use.

\begin{figure}
\centering
AMD Latencies\\
\includegraphics[scale=0.6]{data/amd/latency} \\[3em]
Intel Latencies\\
\includegraphics[scale=0.6]{data/intel/latency}
\caption{
Latency times versus the number of threads on the STREAM benchmark, comparing strided configurations.
Smaller latency times are better.
}
\label{numa:evalLatency}
\end{figure}%

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> related.tex <==
%!TEX root = paper.tex
%
\section{Related work}
\label{sec:related}

\subsection{Collectors} 
As we mentioned in \secref{sec:collector}, our local heap and its treatment bear the most similarities to the minor heaps of the Doligez-Leroy-Gonthier parallel collector~\cite{concurrent-caml-gc,portable-multiprocessor-gc}.
We also perform independent parallel collections of our local heaps.
But, where they perform synchronization upon copying from a full minor heap into their major heap, when our local heap is full, each \vproc{} has a dedicated global heap page that it can copy to without the need for any global synchronization.
Additionally, they use a mark and sweep collector for their major collections, whereas we use a copying collector.

Appel's semi-generational collector~\cite{appel:simple-gc} is also a copying collector.
Unlike our collector, they use multiple global generations and rely on virtual memory hardware to test whether the allocation space has been exhausted.
We have only a single global generation and have not investigated whether a generational approach would further decrease our global collection time.
We decrease the number of free space pointer tests, which is the reason for relying on virtual memory faults on allocation, by coalescing allocation checks within a block of code and performing a single test upon block entry instead of at each allocation point.

In the context of Java, Domani proposed a system that also uses local heaps to allow parallel minor collection~\cite{java-local-heaps}.
But, because they neither had runtime invariants nor did they attempt static analysis, this work relied on validation of every pointer update into global objects to determine whether the object pointed to is a local object.
In that case, the local object needs to be traced and changed into a global object.
In Manticore, local objects only ever become global (outside of garbage collection) if a work-stealing thread attempts to take work from another processor or if a thread passes a message to another processor.
In that case, we know that the object is local and needs to become global, so we promote all of the reachable data from that task, including its closure.

In a similar vein, Steensgaard proposed the use of static escape analysis to partition the allocations into local and possibly global objects~\cite{escape-analysis-thread-heaps}.
This information was then used in his runtime modifications to partition the objects.
Unfortunately, we cannot use such an approach without being hopelessly pessimistic.
Our parallelism is implicit, and many objects, while they could be work-stolen and used by another thread, never are in practice.
We believe that promoting all objects allocated within control-flow reachable from implicitly-threaded parallel constructs would significantly reduce the amount of local heap data allocated.

Like Manticore, the Glasgow Haskell Compiler (GHC) uses a copying generational garbage collector~\cite{multicore-haskell}.
But, their minor (nursery) collections require synchronization and are not independent.
Also, they use no load balancing during their parallel collections, due to decreased performance in both four and seven core configurations.

Anderson recently presented some results for a garbage collector that also uses private nurseries and is targeted at functional languages~\cite{intel-private-heap}.
This work also provides individual threads their own private nurseries, whose memory will never be reassigned, in order to improve locality and cache usage even across minor collections.
They maintain the invariant of no external pointers into the private nurseries through a write barrier, at the expense of 3\% overhead to program execution.
Their concurrent, mark-and-sweep global collector can run concurrently with execution of the program and the nursery allocations.
This concurrent collector cannot currently run in parallel, but that is an explicit design decision because it returns free pages fast enough for practical allocation rates in their benchmarks.
Similar to our work, they saw nearly ideal speedups on dense matrix multiplication.
However, they did not see ideal speedups in their raytracer benchmark and their implementation of Barnes-Hut (which appears to come from the same original source) failed to gain significant speedups past 8 threads.

\paragraph{Dealing with large objects}
Barabash and Petrank propose adding \emph{shortcuts} into large objects such as linked lists or other object graphs to aid in parallel collection~\cite{collector-shortcuts}.
We have not investigated this technique, but we have empirically experienced some of the effects of these objects.
During early collections during a run, when there are relatively few pointers into large objects, we commonly have a situation where there is only one thread performing a global collection and all of the others are blocked waiting for work.
We would like to investigate this strategy, and believe that we could implement it in a lightweight manner by integrating these shortcuts with the per-node global collection lists of available work.

\subsection{Multicore evaluation}
The Java ``allocation wall'' was uncovered by a series of benchmarks run with modern Java virtual machines on the then-available multicore hardware~\cite{allocation-wall}.
This work agrees with ours that in multicore hardware memory issues are a major limiting factor in scaling to multiple processors.
Runtimes and compilers that only take the cache hierarchy into account will encounter issues with memory bus saturation.
However, our results indicate that with locality-aware allocation, scheduling, and collection, there is no reason to believe that there is a fundamental hardware limitation.
Local connections to RAM and the front-side interconnects such as HyperTransport3 are increasing their available bandwidth at a comparable rate to the increase in available cores.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

